FISHing in Uncertainty: Synthetic Contrastive Learning for Genetic Aberration Detection

Detecting genetic aberrations is crucial in cancer diagnosis, typically through fluorescence in situ hybridization (FISH). However, existing FISH image classification methods face challenges due to signal variability, the need for costly manual annotations and fail to adequately address the intrinsic uncertainty. We introduce a novel approach that leverages synthetic images to eliminate the requirement for manual annotations and utilizes a joint contrastive and classification objective for training to account for inter-class variation effectively. We demonstrate the superior generalization capabilities and uncertainty calibration of our method, which is trained on synthetic data, by testing it on a manually annotated dataset of real-world FISH images. Our model offers superior calibration in terms of classification accuracy and uncertainty quantification with a classification accuracy of 96.7% among the 50% most certain cases. The presented end-to-end method reduces the demands on personnel and time and improves the diagnostic workflow due to its accuracy and adaptability. All code and data is publicly accessible at: https://github.com/SimonBon/FISHing

==> sections/setup.tex <==
\section{Experimental Setup}

We implemented our approach using a ResNet-18 backbone, modified to reduce the latent space dimension to 128, and a 64-dimension projection head for contrastive loss training. Classification relied on a 2-layer MLP with 128 features, 0.25 dropout, and ReLU activation. The loss function included a 0.05 temperature, 0.5 for $\lambda$, and 0.01 label smoothing. We used a Cosine Annealing learning rate scheduler with 5 warm-up steps and a 25-epoch cycle, setting learning minimum and maximum at 0.00001 and 0.001 respectively, and a batch size of 128. Two augmentation grades were tested: heavy (\textit{Ours Heavy}) and light (\textit{Ours Light}).
\vspace{4pt}

\noindent \textbf{Baselines}: \textit{bigFISH} \cite{Imbert2022} and a pretrained spot detection RetinaNet model from \cite{Gutwein2024}, with a classification head fine tuned on our synthetic training datasets. Another baseline, \textit{ResNet18+CE}, used a ResNet-18 backbone with cross-entropy loss, mirroring our training parameters.  We further compared against two CL baselines, \textit{CL+Detached} and \textit{CL+Attached}, which utilize the same ResNet-18 architecture as our \textit{Ours Heavy} and \textit{Ours Light} methods. These baselines differ in their training strategy: \textit{CL+Detached} maintains a frozen backbone, while \textit{CL+Attached} allows for backbone fine-tuning during classifier training.
% (optimized for signal detection with log\_kernel\_size of 2 in both x and y directions and a minimum distance of 2 in x and y and 0.0002 threshold) 

